Optimal Transport for Unsupervised Hallucination Detection in Neural Machine Translation

Neural machine translation (NMT) has become the de-facto standard in real-world machine translation applications. However, NMT models can unpredictably produce severely pathological translations, known as hallucinations, that seriously undermine user trust. It becomes thus crucial to implement effective preventive strategies to guarantee their proper functioning. In this paper, we address the problem of hallucination detection in NMT by following a simple intuition: as hallucinations are detached from the source content, they exhibit encoder-decoder attention patterns that are statistically different from those of good quality translations. We frame this problem with an optimal transport formulation and propose a fully unsupervised, plug-in detector that can be used with any attention-based NMT model. Experimental results show that our detector not only outperforms all previous model-based detectors, but is also competitive with detectors that employ large models trained on millions of samples.

==> legacy_text.tex <==
% \section{\textsc{Info--Attention}}
% Anomalous attention maps have been connected to the hallucinatory mode in several works~\citep{lee2018hallucinations, raunak-etal-2021-curious, guerreiroetal2022}. Our method builds on this idea and uses the Wasserstein distance to estimate the cost of transforming a translation source mass distribution into a reference distribution. Intuitively, the higher the cost of such transformation, the more distant -- and hence more anomalous -- the attention of such translation is with respect to the attention of that reference translation. Importantly, our method is fully unsupervised and only requires model-based information that is easily obtained as a by-product of generating a translation.

% \subsection{\textsf{Wass-to-Unif}: scoring function $s_{\textsf{wtu}}$} Our first scoring function $s_{\textsf{wtu}}$ is inspired by the observation made in~\citet{guerreiroetal2022}: attention maps for which the source attention mass is highly concentrated on a very sparse set of tokens can be highly predictive of hallucinations. 

% \paragraph{Choice of distance function.}  We consider a distance function that guarantees that the cost of transporting a unit mass from token $i$ to token $j \neq i$ is constant -- $d(i,j) = m_{ij}$, where $\bm{M} = \bm{J}_n - \bm{I}_n$, where $\bm{J}_n = \bm{1} \bm{1}^\top$, $\bm{1} \in \mathbb{R}^n$. We show that for this distance function, solving for the Wasserstein distance (see Equation~\ref{eq:wass_dist}) is the following linear program (see Appendix for a proof):
% \begin{equation}\label{eq:wass_dist_uni}
% \begin{split}
%     \max_{\bm{\gamma} \in \Pi(\bm{\mu}, \bm{\nu})} & \mathrm{tr}(\bm{\gamma})\\
%   \text{s.t} \quad & \bm{\gamma} \bm{1} = \bm{\mu}, \bm{\gamma}^\top \bm{1} = \bm{\nu},  \bm{\gamma} \geq 0
%   \end{split}
% \end{equation}
% Thus, on this metric space, the Wasserstein distance depends solely on the probability mass that is transported to transform $\bm{\mu}$ to $\bm{\nu}$, thus ignoring the starting locations and destinations of that probability mass. This design choice reflects the observation in~\cite{guerreiroetal2022}: attention maps that were predictive of hallucinations had source mass highly concentrated on a sparse set of tokens, regardless of their location in the source sentence.

% \paragraph{Choice of reference distribution.} For a test sample $\bm{x}\in \mathbb{R}^n$, we consider the uniform distribution $\bm{u} \in \mathbb{R}^n$ as the reference distribution~-- $\bm{u} = \frac{1}{n} \cdot \bm{1}, \bm{1} \in \mathbb{R}^n$ -- as, by definition, a uniform source mass distribution guarantees that all tokens are attended to. Thus, the bigger the Wasserstein distance between the attention distribution of a test sample and the uniform distribution, the more peaked the former is, and the closer it is to a map that is highly predictive of hallucinations~\citep{raunak-etal-2021-curious, guerreiroetal2022}.

% % \begin{equation}
% %     \begin{cases}
% %     \max_{\bm{\gamma} \in \Pi(\bm{\mu}, \bm{\nu})} \mathrm{tr}(\bm{\gamma})\\
% %     \bm{\gamma} \bm{1} = \bm{\mu}\\
% %     \bm{\gamma}^\top \bm{1} = \bm{\nu}\\
% %     \bm{\gamma} \geq 0
% %     \end{cases}
% %     \label{eq:wass_dist_uni}
% % \end{equation}

% \paragraph{Scoring.} For a test sample $\bm{x}$, we obtain $\bm{\phi}(\bm{x})\in \mathbb{R}^n$ and compute
% \begin{equation}
% s_{\textsf{wtu}}(\bm{x}) = W(\bm{\phi}(\bm{x}), \bm{u})
% \end{equation}
% by solving Equation~\ref{eq:wass_dist_uni}. 

% \subsection{\textsf{Wass-to-Data}: scoring function $s_{\textsc{WTD}}$} Hallucinations, contrary to good translations, are not fully supported by the source content. We hypothesize that hallucinations exhibit encoder-decoder attention patterns that are different from those found in other translations. Thus, in our second scoring function, $s_{\textsc{WTD}}$, we aim to find translations whose source attention mass distribution is distant from those obtained by the same model for a set of reference translations. 

% \paragraph{Choice of distance function.}  We use the absolute value function as the distance function $d$. This constrasts with the choice of distance function in $s_{\textsc{Unif}}$, since the cost of transporting a unit mass from token $i$ to token $j$ is not constant, and instead proportional to $|i-j|$. 

% \paragraph{Choice of reference distribution.} Differently to $s_{\textsc{Unif}}$, instead of considering a single distribution as the reference distribution, we will compute the Wasserstein distance between $\bm{\phi}(\bm{x})$ and every single distribution contained in a set of reference source mass distributions obtained with the same model, $\mathcal{R}$. To construct $\mathcal{R}$, we use an heldout dataset $\mathcal{D}_{\textrm{held}}$ that contains samples for which the model generates good quality translations, and the set of source mass distributions generated by the model for the samples in $\mathcal{D}_{\textrm{held}}$, $\mathcal{R}_{\textrm{held}} = \{\bm{x} \in \mathcal{D}_{\textrm{held}}: \bm{\phi}(\bm{x})\}$. As it is computationally expensive to have $\mathcal{R} = \mathcal{R}_{\textrm{held}}$ when $|\mathcal{D}_{\textrm{held}}|$ is large, we set the maximum cardinality of set $\mathcal{R}$, $|\mathcal{R}|_{\textrm{max}}$, and restrict $\mathcal{R}$ to contain at most $|\mathcal{R}|_{\textrm{max}}$ distributions in $\mathbb{R}^m$, with $m \in [(1-\delta) n, (1+\delta) n]$ for a predefined $\delta \in ]0,1[$.\footnote{If $\mathcal{R}$ contains more than $|\mathcal{R}|_{\textrm{max}}$ samples, we restrict its cardinality to $|\mathcal{R}|_{\textrm{max}}$ by randomly sampling $|\mathcal{R}|_{\textrm{max}}$ samples and discarding the rest.} 

% % \begin{algorithm}[ht]
% % 	\caption{Selection of $\mathcal{R}$}
% % 	\label{alg:exmp}
% % 	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
% % 	\renewcommand{\algorithmicensure}{\textbf{Output:}}
% % 	\begin{algorithmic}[1]
% % 		\REQUIRE Test sample source length $n$, set of source mass distributions generated by the model for samples in $\mathcal{D}_{\textrm{held}}$, $\mathcal{R}_{\textrm{held}}$
% % 		\STATE Obtain $\mathcal{R}_1 = \{\bm{x} \in \mathcal{D}_{\textrm{held}}: |\bm{x}| = n\}$;
% % 		\STATE Obtain $\mathcal{R}_2 = \{\bm{x} \in \mathcal{D}_{\textrm{held}}: |\bm{x}| \in [(1-\delta) n, (1+\delta) n]$
% % 		\IF{$|\mathcal{R}_1| \geq |\mathcal{R}|_{\textrm{max}}$}
% % 			\STATE Set $\mathcal{R}$ to contain $|\mathcal{R}|_{\textrm{max}}$ random samples from $\mathcal{R}_1$
% % 		\ELSE
% % 			\STATE Obtain $\mathcal{R}_2 = \{\bm{x} \in \mathcal{D}_{\textrm{held}}: |\bm{x}| \in [(1-\delta) n, (1+\delta) n]$ \\
			
% % 		\ENDIF
% % 		\ENSURE set of reference distributions $\mathcal{R}$
% % 	\end{algorithmic}
% % \end{algorithm}




% \paragraph{Scoring.} For a test sample $\bm{x}$, we obtain $\bm{\phi}(\bm{x})\in \mathbb{R}^n$ and the set of reference distributions $\mathcal{R}$, and compute pairwise Wasserstein distances between $\bm{\phi}(\bm{x})$ and each element of $\mathcal{R}$:
% \pierre{I find $\mathbb{W}$ super fancy but you used round notations for set ? what about $\mathbb{W}$  for wasserstein and mathcla. for sets ? }
% \begin{equation}
% \mathbb{W}_{\textsf{wtd}}(\bm{x}) = \{\bm{x}' \in \mathcal{R}: W(\bm{\phi}(\bm{x}), \bm{\phi}(\bm{x}'))\}
% \end{equation}
% Finally, we aggregate the $|\mathcal{R}|$ scores by averaging the bottom-$k$ distances:
% \begin{equation}
%     s_{\textsf{wtd}}(\bm{x}) = \frac{1}{k} \sum_{i=1}^{k} \min_{(k)} \mathbb{W}_{\textsf{wtd}}(\bm{x})
% \end{equation}
% where $\min_{(k)}(A)$ is a set containing the bottom-$k$ elements of $A$. \pierre{$\mathcal{A}$?}

% \subsection{\textsf{Wass-Combo}: scoring function $s_{\textsc{WC}}$}
% In this scoring function, we aim to combine \textsf{Wass-to-Unif} and \textsf{Wass-to-Data} into a single detector. To do so, we propose using a two-staged process that exploits the computational benefits of \textsf{Wass-to-Unif} over \textsf{Wass-to-Data}. Put simply, (i)~we start by assessing whether a test sample is deemed an hallucination according to \textsf{Wass-to-Unif}, and if not (ii)~we compute the \textsf{Wass-to-Data} score. 

% \paragraph{Scoring.} For a test sample $\bm{x}$, we obtain $\bm{\phi}(\bm{x})\in \mathbb{R}^n$ and compute:
% \begin{align}
%     s_{\textsf{wc}}(\bm{x}) = \mathbbm{1} &\left[s_{\textsf{wtu}}(\bm{x}) > \tau \right] \times s_{\textsf{wtu}}(\bm{x}) \\ &+ \mathbbm{1} \left[s_{\textsf{wtu}}(\bm{x}) \leq \tau \right] \times s_{\textsf{wtd}}(\bm{x}) \nonumber
% \end{align}
% for a predefined scalar threshold $\tau$. To set that threshold, we note that, for in-domain settings, previous work reported hallucinatory rates of~$0{.}2$ to $2\%$~\citep{muller-etal-2020-domain, xiao-wang-2021-hallucination, salted_raunak2022}. Thus, we compute~$\mathbb{W}_{\textsf{wtu}} = \{\bm{x} \in \mathcal{D}_{\textrm{held}}: s_{\textsf{wtu}} (\bm{x})\}$ and set $\tau=P_{K}$, i.e $\tau$ is the $K-$th percentile of $\mathbb{W}_{\textsf{wtu}}$ with $K \in\, ]98,100[$.
 
% considering the uniform distribution as the reference distribution. By definition, a uniform source mass distribution guarantees that all tokens are attended to. 

%For in-domain settings, previous work reported hallucinatory rates of~$0{.}2-2\%$~\citep{muller-etal-2020-domain, xiao-wang-2021-hallucination, salted_raunak2022}. 


% \textsf{COMET}       & \multicolumn{1}{r}{83.42} & \multicolumn{1}{r}{58.46}  \\


% \begin{table*}[t]
% \centering
% \footnotesize
% \renewcommand\arraystretch{1.05}
% \begin{tabular}{>{\arraybackslash}m{1.85cm} c c c c}
% \toprule
% \multirow{ 2}{*}{\textsc{Detector}}  & \multirow{ 2}{*}{{\textbf{\textsc{All}}}} & \textbf{Fully} & \multirow{ 2}{*}{{\textbf{Oscillatory}}} & {\textbf{Strongly}} \\
% & & \textbf{Detached} & & \textbf{Detached} \\
% \midrule
% \textsf{COMET-QE}       & 57.24 & 54.50 & \textbf{34.70} & 73.90  \\
% \textsf{Attn-ign-SRC}   & 72.83 & 8.51 & 81.24 & 76.68 \\
% \textsf{Seq-Logprob}    & 59.02 & 4.62 & 72.99 & \textbf{65.39} \\ \midrule \midrule  
% \textbf{\textit{Our Methods}} &  &  \\
% $s_{\textsc{Unif}}$ & 72.22 & \textbf{3.27} & 78.78 & 88.32 \\
% $s_{\textsc{PWC}}$ & \textbf{48.15} \scriptsize{\textcolor{gray}{$\pm$ 0.54}} & 36.60 \scriptsize{\textcolor{gray}{$\pm$ 1.92}} & 40.04 \scriptsize{\textcolor{gray}{$\pm$ 1.57}} & \textbf{63.96} \scriptsize{\textcolor{gray}{$\pm$ 2.04}} \\
% $s_{\textsc{Combo}}$ & \textbf{47.56} \scriptsize{\textcolor{gray}{$\pm$ 1.30}} & 3.56 \scriptsize{\textcolor{gray}{$\pm$ 0.00}} & 41.38 \scriptsize{\textcolor{gray}{$\pm$ 1.59}} & \textbf{64.55} \scriptsize{\textcolor{gray}{$\pm$ 1.93}}\\
% \bottomrule
% \end{tabular}
% \label{tab:static_error_table}
% \caption{Performance according to FPR@90TPR of the hallucination detectors. The lower the better. }
% \end{table*}
